Detailed dust modelling in the L-Galaxies semi-analytic model of galaxy formation

We implement a detailed dust model into the L-Galaxies semi-analytical model which includes: injection of dust by type II and type Ia supernovae (SNe) and AGB stars; grain growth in molecular clouds; and destruction due to supernova-induced shocks, star formation, and reheating. Our grain growth model follows the dust content in molecular clouds and the inter-cloud medium separately, and allows growth only on pre-existing dust grains. At early times, this can make a significant difference to the dust growth rate. Above $z\sim8$, type II SNe are the primary source of dust, whereas below $z\sim8$, grain growth in molecular clouds dominates, with the total dust content being dominated by the latter below $z\sim6$. However, the detailed history of galaxy formation is important for determining the dust content of any individual galaxy. We introduce a fit to the dust-to-metal (DTM) ratio as a function of metallicity and age, which can be used to deduce the DTM ratio of galaxies at any redshift. At $z\lesssim3$, we find a fairly flat mean relation between metallicity and the DTM, and a positive correlation between metallicity and the dust-to-gas (DTG) ratio, in good agreement with the shape and normalisation of the observed relations. We also match the normalisation of the observed stellar mass -- dust mass relation over the redshift range of $0-4$, and to the dust mass function at $z=0$. Our results are important in interpreting observations on the dust content of galaxies across cosmic time, particularly so at high redshift.

==> first.tex <==
\section{The first galaxies}\label{sec:firstGalaxies}

\begin{figure*}
	\begin{center}
		\includegraphics[width=0.32\textwidth]{./Figures/z9_12DTM_stellar_MR_MRII_median}
		\includegraphics[width=0.32\textwidth]{./Figures/z9_12Dust_Stellar_MR_MRII_median}	
		\includegraphics[width=0.32\textwidth]{./Figures/z9_12dust_prod_rate_redshift_MR_full}
		\caption{The DTM-stellar mass relation (first panel),
                  stellar-dust relation (second panel) and the dust production
                  rates (third panel) for z = 9 to z = 12, the redshift range
                  where we may potentially find the first galaxies using
                  JWST.  The errorbars denote the 84 and 16
                  percentiles.}
		\label{fig:first_gals}
	\end{center}
\end{figure*}

\peter{Relly not obvious to me that this section adds very much, but leave it
  for now.}
  \robc{Agreed. Unless Stephen can think of something exciting to add here, we may as well remove this section, and consider a very-high-redshift paper another time.}

In this section we will focus on the dust content of the highest redshift
galaxies (z $\ge$ 9). These, which are some of the first galaxies in the
Universe, and which will hopefully be detected by the James Webb Space Telescope (JWST) in
the next few years, could potentially have very different dust properties to the
observations we have compared the model to so far.

Figure~\ref{fig:first_gals} shows the $M_{*}$ -- DTM relation, the $M_{*}$ --
$M\sub{dust}$ relation, and the dust production rates for our model from $z =
12$ to 9. We see that \tTwo\ supernovae dominate the production of dust at very
early times. Thus, at the highest redshifts, the dispersion in the DTM ratio is
small, and the $M_*$ -- $M\sub{dust}$ relation doesn't evolve. Although the
median DTM ratio increases only slightly from $z=12$ to 9, the dispersion
increases rapidly as grain growth takes over at $z<8$. \robc{There must be some
  observed dusty quasars at $z \gtrsim 6$ or something to which we can
  compare. That CR7 galaxy, for example? Stephen Wilkins should know of
  some\ldots{}}


